The Online Observation Quality System Software Architecture for the ASTRI Mini-Array Project

The ASTRI Mini-Array is an international collaboration led by the Italian National Institute for Astrophysics. This project aims to construct and operate an array of nine Imaging Atmospheric Cherenkov Telescopes to study gamma-ray sources at very high energy (TeV) and perform stellar intensity interferometry observations. We describe the software architecture and the technologies used to implement the Online Observation Quality System (OOQS) for the ASTRI Mini-Array project. The OOQS aims to execute data quality checks on the data acquired in real-time by the Cherenkov cameras and intensity interferometry instruments, and provides feedback to both the Central Control System and the Operator about abnormal conditions detected. The OOQS can notify other sub-systems, triggering their reaction to promptly correct anomalies. The results from the data quality analyses (e.g. camera plots, histograms, tables, and more) are stored in the Quality Archive for further investigation and they are summarised in reports available to the Operator. Once the OOQS results are stored, the operator can visualize them using the Human Machine Interface. The OOQS is designed to manage the high data rate generated by the instruments (up to 4.5 GB/s) and received from the Array Data Acquisition System through the Kafka service. The data are serialized and deserialized during the transmission using the Avro framework. The Slurm workload scheduler executes the analyses exploiting key features such as parallel analyses and scalability.

==> bib_bkp.tex <==


@INPROCEEDINGS{2016JPhCS.718e2028P,
       author = {{Pareschi}, Giovanni and {Bonnoli}, Giacomo and {Vercellone}, Stefano and {ASTRI Collaboration} and {CTA Consortium}},
        title = "{The mini-array of ASTRI SST-2M telescopes, precursors for the Cherenkov Telescope Array}",
    booktitle = {Journal of Physics Conference Series},
         year = 2016,
       series = {Journal of Physics Conference Series},
       volume = {718},
        month = may,
          eid = {052028},
        pages = {052028},
          doi = {10.1088/1742-6596/718/5/052028},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016JPhCS.718e2028P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Krennrich_2009,
	doi = {10.1088/1367-2630/11/11/115008},
	url = {https://doi.org/10.1088/1367-2630/11/11/115008},
	year = 2009,
	month = {nov},
	publisher = {{IOP} Publishing},
	volume = {11},
	number = {11},
	pages = {115008},
	author = {Frank Krennrich},
	title = {Gamma ray astronomy with atmospheric Cherenkov telescopes: the future},
	journal = {New Journal of Physics},
	abstract = {Atmospheric Cherenkov telescopes have been key to the recent discoveries in teraelectronvolt (TeV) γ-ray astronomy. The detection of TeV γ rays from more than 90 galactic and extragalactic sources provides a wealth of data for probing physical phenomena that pertain to some of the big questions in astrophysics. These include the understanding of the origin of cosmic rays, unveiling the connection between relativistic jets and black holes, shedding light on dark matter and its relation to supersymmetric particles and estimating the brightness of cosmological diffuse radiation fields in the optical/infrared waveband. While these recent advances were made with instruments designed in the 1990s, the present paper is concerned with a next generation of imaging atmospheric Cherenkov telescopes (IACTs) that are currently in the conceptual planning stage. We discuss the basic ideas, the required technology and expected performance of a ⩾1 square-kilometer array, which is poised to yield the most dramatic step yet to come in TeV astronomy.}
}


@INPROCEEDINGS{2018SPIE10702E..37C,
       author = {{Catalano}, Osvaldo and {Capalbi}, Milvia and {Gargano}, Carmelo and {Giarrusso}, Salvo and {Impiombato}, Domenico and {La Rosa}, Giovanni and {Maccarone}, Maria Concetta and {Mineo}, Teresa and {Russo}, Francesco and {Sangiorgi}, Pierluca and {Segreto}, Alberto and {Sottile}, Giuseppe and {Biondo}, Benedetto and {Bonanno}, Giovanni and {Garozzo}, Salvatore and {Grillo}, Alessandro and {Marano}, Davide and {Romeo}, Giuseppe and {Scuderi}, Salvatore and {Canestrari}, Rodolfo and {Conconi}, Paolo and {Giro}, Enrico and {Pareschi}, Giovanni and {Sironi}, Giorgia and {Conforti}, Vito and {Gianotti}, Fulvio and {Gimenes}, Renato},
        title = "{The ASTRI camera for the Cherenkov Telescope Array}",
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy VII},
         year = 2018,
       editor = {{Evans}, Christopher J. and {Simard}, Luc and {Takami}, Hideki},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {10702},
        month = jul,
          eid = {1070237},
        pages = {1070237},
          doi = {10.1117/12.2314984},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018SPIE10702E..37C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2019arXiv190905409L,
       author = {{Leite}, Leonardo and {Rocha}, Carla and {Kon}, Fabio and {Milojicic}, Dejan and {Meirelles}, Paulo},
        title = "{A Survey of DevOps Concepts and Challenges}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Software Engineering, D.2, D.2},
         year = 2019,
        month = sep,
          eid = {arXiv:1909.05409},
        pages = {arXiv:1909.05409},
archivePrefix = {arXiv},
       eprint = {1909.05409},
 primaryClass = {cs.SE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190905409L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2002SPIE.4848...43C,
       author = {{Chiozzi}, Gianluca and {Gustafsson}, Birger and {Jeram}, Bogdan and {Plesko}, Mark and {Sekoranja}, Matej and {Tkacik}, Gasper and {Zagar}, K.},
        title = "{CORBA-based Common Software for the ALMA project}",
    booktitle = {Advanced Telescope and Instrumentation Control Software II},
         year = 2002,
       editor = {{Lewis}, Hilton},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {4848},
        month = dec,
        pages = {43-54},
          doi = {10.1117/12.461036},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002SPIE.4848...43C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2021ICRCIovenitti,
    author = {{Iovenitti}, Simone and {Sironi}, Giorgia and {Catalano}, Osvaldo and {Segreto}, Alberto and {Mineo}, Teresa},
        title = "Effective pointing of the ASTRI-Horn telescope using the Cherenkov camera with the Variance method",
    booktitle = {37th International Cosmic Ray Conference (ICRC2021)},
         year = 2021,
       series = {International Cosmic Ray Conference},
        volume = {This Proceeding}
}

@inproceedings{Antonelli:2021ml,
  author = "Antonelli, Lucio Angelo",
  title = "{The ASTRI Mini-Array at Teide Observatory}",
  doi = "10.22323/1.395.0897",
  booktitle = "Proceedings of 37th International Cosmic Ray Conference {\textemdash} PoS(ICRC2021)",
  year = 2021,
  volume = "395",
  pages = "897"
}


@inproceedings{Incardona2022,
author = {Incardona, Federico  and  Costa, Alessandro and  Munari, Kevin  and  Gambadoro , Salvatore and Bruno, Pietro and Bulgarelli Andrea, and Germani, Stefano and Gianotti, Fulvio and Grillo, Alessandro and Russo , Federico and Schwarz , Joseph and Tosti , Gino and Cavalieri, Salvatore},
title = {{The Monitoring Logging and Alarm System of the ASTRI Mini-Array gamma-ray air-Cherenkov experiment at the Observatorio del Teide}},
volume = {Proc. of SPIE 12189},
booktitle = {Software and Cyberinfrastructure for Astronomy VII},
editor = {Jorge Ibsen, Gianluca Chiozzi},
year = {2022},
}

@inproceedings{Corpora2022,
author = {Corpora, Mattia  and  Grillo, Alessandro  and  Sangiorgi, Pierluca  and  Capalbi, Milvia  and  Catalano, Osvaldo  and  Sottile, Giuseppe  and  Tosti, Gino  and  Bulgarelli, Andrea  and  Lucarelli, Fabrizio  and  Parmiggiani, Nicolò  and  Schwarz, Joseph Hilary  and  Russo, Federico  and  Scuderi, Salvatore},
title = {{Design and development of the Supervisor Software Component for the ASTRI Mini-Array Cherenkov Camera}},
volume = {Proc. of SPIE 12189},
booktitle = {Software and Cyberinfrastructure for Astronomy VII},
editor = {Jorge Ibsen, Gianluca Chiozzi},
year = {2022},
}


@inproceedings{Conforti2022,
author = {Conforti , Vito and Gianotti , Fulvio and Pastore, Valerio and Trifoglio, Massimo and Bulgarelli, Andrea and Addis, Antonio, and Baroncelli , Leonardo, and Capalbi , Milvia and Fioretti, Valentina and Parmiggiani, Nicolò and Sangiorgi, Pierluca and Catalano , Osvaldo and Costa , Alessandro and Incardona Federico and Russo, Federico},
title = {{The Array Data Acquisition System software architecture of the ASTRI Mini-Array Project}},
volume = {Proc. of SPIE 12189},
booktitle = {Software and Cyberinfrastructure for Astronomy VII},
editor = {Jorge Ibsen, Gianluca Chiozzi},
year = {2022},
}

@inproceedings{Corpora:2021Oh,
  author = "Corpora, Mattia  and  Grillo, Alessandro  and  Sangiorgi, Pierluca  and  Capalbi, Milvia  and  Catalano, Osvaldo  and  Sottile, Giuseppe  and  Russo, Federico  and  Tosti, Gino  and  Bulgarelli, Andrea  and  Lucarelli, Fabrizio  and  Parmiggiani, Nicolò  and  Schwarz, Joseph  and  Russo, Francesco  and  Scuderi, Salvatore",
  title = "{The Architecture of ASTRI Mini Array Cherenkov Camera Software Supervisor}",
  doi = "10.22323/1.395.0691",
  booktitle = "Proceedings of 37th International Cosmic Ray Conference {\textemdash} PoS(ICRC2021)",
  year = 2021,
  volume = "395",
  pages = "691"
}




@inproceedings{Costa:2021c8,
  author = "Costa, Alessandro  and  Munari, Kevin  and  Incardona, Federico  and  Bruno, Pietro Giuseppe  and  Germani, Stefano  and  Grillo, Alessandro  and  Oya, Igor  and  Sciacca, Eva  and  Becciani, Ugo  and  Raciti, Mario",
  title = "{The Monitoring, Logging, and Alarm system for the Cherenkov Telescope Array}",
  doi = "10.22323/1.395.0700",
  booktitle = "Proceedings of 37th International Cosmic Ray Conference {\textemdash} PoS(ICRC2021)",
  year = 2021,
  volume = "395",
  pages = "700"
}
    
@inproceedings{Bulgarelli2022,
author = {Bulgarelli , Andrea and Lucarelli , Fabrizio and Tosti, Gino and Conforti , Vito and Parmiggiani , Nicolò and Schwarz , Joseph Hilary and Antonelli, Lucio Angelo and Baroncelli , Leonardo and Bigongiari, Ciro and Capalbi, Milvia and Cardillo, Martina and Rodriguez Castillo , Guillermo Andres and Catalano, Osvaldo and Compagnino , Antonio Alessio and Corpora, Mattia and Costa, Alessandro and Crestan, Silvia and Cusumano , Giancarlo and D'Aì , Antonino and Fioretti, Valentina and Gallozzi , Stefano and Germani, Stefano and Gianotti , Fulvio and Giordano , Valentina and Giuliani, Andrea and Bruno, Pietro Giuseppe and Green , Jarred Gershon and Grillo,  Alessandro and Incardona , Federico and Iovenitti, Simone and La Palombara, Nicola and La Parola, Valentina and Landoni, Marco and Lombardi, Saverio and Maccarone, Maria Concetta and Millul, Rachele and Mineo, Teresa and Mollica, Davide and Pagliaro, Antonio and Pareschi, Giovanni and Pastore, Valerio and Perri, Matteo and Pintore, Fabio and Romano, Patrizia and Russo, Federico and Sangiorgi, Pierluca and Saturni, Francesco Gabriele and Sciacca, Eva and Scuderi, Salvatore, and Tacchini, Alessandro and Testa, Vincenzo and Trifoglio, Massimo and Tutone, Antonio and Vercellone, Stefano},
title = {{The Software Architecture and development approach for the ASTRI Mini-Array gamma-ray air-Cherenkov experiment at the Observatorio del Teide}},
volume = {Proc. of SPIE 12189},
booktitle = {Software and Cyberinfrastructure for Astronomy VII},
editor = {Jorge Ibsen, Gianluca Chiozzi},
year = {2022},
}
    
@ARTICLE{2008NIMPA.588...52T,
       author = {{Tavani}, M. and others},
        title = "{The AGILE space mission}",
      journal = {Nuclear Instruments and Methods in Physics Research A},
         year = 2008,
        month = apr,
       volume = {588},
       number = {1-2},
        pages = {52-62},
          doi = {10.1016/j.nima.2008.01.023},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008NIMPA.588...52T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...502..995T,
       author = {{Tavani}, M. and others},
        title = "{The AGILE Mission}",
      journal = {\aap},
     keywords = {instrumentation: detectors, techniques: high angular resolution, techniques: image processing, gamma rays: observations, X-rays: general, Astrophysics},
         year = 2009,
        month = aug,
       volume = {502},
       number = {3},
        pages = {995-1013},
          doi = {10.1051/0004-6361/200810527},
archivePrefix = {arXiv},
       eprint = {0807.4254},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...502..995T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@inproceedings{10.1117/12.2530896,
author = {Enrico Giro and Rodolfo Canestrari and Pietro Bruno and Osvaldo Catalano and Dino Fugazza and Nicola La Palombara and Maria Concetta Maccarone and Giovanni Pareschi and Federico Russo and Salvatore Scuderi and Alberto Segreto and Giorgia Sironi and Gino Tosti and G. Marchiori and A. Busatta and E. Marcuzzi and I. Folla},
title = {{The ASTRI-Horn telescope validation toward the production of the ASTRI Mini-Array: a proposed pathfinder for the Cherenkov Telescope Array}},
volume = {11119},
booktitle = {Optics for EUV, X-Ray, and Gamma-Ray Astronomy IX},
editor = {Stephen L. O'Dell and Giovanni Pareschi},
organization = {International Society for Optics and Photonics},
publisher = {SPIE},
pages = {446 -- 460},
keywords = {Cherenkov Telescope, ASTRI, CTA, imaging atmospheric Cherenkov telescope, very high-energy gamma rays, Schwarzschild-Couder telescopes, slumped glass mirrors},
year = {2019},
doi = {10.1117/12.2530896},
URL = {https://doi.org/10.1117/12.2530896}
}


@article{IOVENITTI_CAMERA_ALIGNMENT,
	title = {Assessment of the {Cherenkov} camera alignment through {Variance} images for the {ASTRI} telescope},
	volume = {53},
	issn = {1572-9508},
	url = {https://rdcu.be/cALxv},
	doi = {doi.org/10.1007/s10686-021-09814-9},
	abstract = {A peculiar aspect of Cherenkov telescopes is that they are designed to detect atmospheric light flashes on the time scale of nanoseconds, being almost blind to stellar sources. As a consequence, the pointing calibration of these instruments cannot be done in general exploiting the standard astrometry of the focal plane. In this paper we validate a procedure to overcome this problem for the case of the innovative ASTRI telescope, developed by INAF, exploiting sky images produced as an ancillary output by its novel Cherenkov camera. In fact, this instrument implements a statistical technique called “Variance method” (VAR) owning the potentiality to image the star field (angular resolution \${\textbackslash}sim 11{\textasciicircum}\{{\textbackslash}prime \}\$). We demonstrate here that VAR images can be exploited to assess the alignment of the Cherenkov camera with the optical axis of the telescope down to \${\textbackslash}sim 1\{{\textasciicircum}\{{\textbackslash}prime {\textbackslash}prime \}\}\$. To this end, we evaluate the position of the stars with sub-pixel precision thanks to a deep investigation of the convolution between the point spread function and the pixel distribution of the camera, resulting in a transformation matrix that we validated with simulations. After that, we considered the rotation of the field of view during long observing runs, obtaining light arcs that we exploited to investigate the alignment of the Cherenkov camera with high precision, in a procedure that we have already tested on real data. The strategy we have adopted, inherited from optical astronomy, has never been performed on Variance images from a Cherenkov telescope until now, and it can be crucial to optimize the scientific accuracy of the incoming MiniArray of ASTRI telescopes.},
	language = {en},
	number = {1},
	urldate = {2021-11-04},
	journal = {Experimental Astronomy},
	author = {Iovenitti, Simone and Sironi, Giorgia and Giro, Enrico and Segreto, Alberto and Catalano, Osvaldo and Capalbi, Milvia},
	month = nov,
	year = {2021},
	pages = {117--132},
	file = {Springer Full Text PDF:/Users/simo/Software/LaTeX/Zotero/storage/IJXX9A4D/Iovenitti et al. - 2021 - Assessment of the Cherenkov camera alignment throu.pdf:application/pdf},
}

@ARTICLE{2021arXiv210508648B,
       author = {{Baroncelli}, Leonardo and {Bulgarelli}, Andrea and {Parmiggiani}, Nicolo and {Fioretti}, Valentina and {Addis}, Antonio and {De Cesare}, Giovanni and {Di Piano}, Ambra and {Conforti}, Vito and {Gianotti}, Fulvio and {Russo}, Federico and {Maurin}, Gilles and {Vuillaume}, Thomas and {Aubert}, Pierre and {Garcia}, Emilio and {Zoccoli}, Antonio},
        title = "{rta-dq-lib: a software library to perform online data quality analysis of scientific data}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.08648},
        pages = {arXiv:2105.08648},
archivePrefix = {arXiv},
       eprint = {2105.08648},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210508648B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@inproceedings{Zampieri2022,
author = {Zampieri, Luca and Bonanno, Giovanni and Bruno, Pietro and Gargano, Carmelo and Lessio, Luigi and Naletto, Giampiero and Paoletti, Lorenzo and Rodeghiero, Gabriele and Romeo, Giuseppe and Bulgarelli, Andrea and Conforti, Vito and Fiori, Michele and Gallozzi, Stefano and Ganotti, Fulvio and Grillo, Alessandro and Landoni, Marco and Lombardi, Saverio and Lucarelli, Fabrizio and Morselli, Aldo and Occhipinti, Giovanni and Parmiggiani, Nicolò and Pernechele, Claudio and Rodriguez Fernandez, Gonzalo and Russo, Federico and Sironi, Giorgia and Timpanaro, Maria Cristina and Giordano, Valentina and Pareschi, Giovanni and Scuderi, Salvatore and Tosti, Gino},
title = {{A Stellar Intensity Interferometry Instrument for the ASTRI Mini-Array telescopes}},
volume = {Proc. of SPIE 12183},
booktitle = {Optical and Infrared Interferometry and Imaging VIII},
editor = {Antoine Mérand, Stephanie Sallum, Joel Sanchez-Bermudez},
year = {2022},
}

@inproceedings{Pastore2022,
author = {Pastore, V. and et al.},
title = {{Array Data Acquisition System interface for online distribution of acquired data in the ASTRI Mini-Array project}},
volume = {Proc. of SPIE 12189},
booktitle = {Software and Cyberinfrastructure for Astronomy VII},
editor = {Jorge Ibsen, Gianluca Chiozzi},
year = {2022},
}
